Grounding Stylistic Domain Generalization with Quantitative Domain Shift Measures and Synthetic Scene Images

Domain Generalization (DG) is a challenging task in machine learning that requires a coherent ability to comprehend shifts across various domains through extraction of domain-invariant features. DG performance is typically evaluated by performing image classification in domains of various image styles. However, current methodology lacks quantitative understanding about shifts in stylistic domain, and relies on a vast amount of pre-training data, such as ImageNet1K, which are predominantly in photo-realistic style with weakly supervised class labels. Such a data-driven practice could potentially result in spurious correlation and inflated performance on DG benchmarks. In this paper, we introduce a new DG paradigm to address these risks. We first introduce two new quantitative measures ICV and IDD to describe domain shifts in terms of consistency of classes within one domain and similarity between two stylistic domains. We then present SuperMarioDomains (SMD), a novel synthetic multi-domain dataset sampled from video game scenes with more consistent classes and sufficient dissimilarity compared to ImageNet1K. We demonstrate our DG method SMOS. SMOS first uses SMD to train a precursor model, which is then used to ground the training on a DG benchmark. We observe that SMOS contributes to state-of-the-art performance across five DG benchmarks, gaining large improvements to performances on abstract domains along with on-par or slight improvements to those on photo-realistic domains. Our qualitative analysis suggests that these improvements can be attributed to reduced distributional divergence between originally distant domains. Our data are available at https://github.com/fpsluozi/SMD-SMOS .

==> draft/iccv_new_abstract.tex <==
Image domains in previous Domain Generalization (DG) benchmarks have been sampled out of only apparently distinguishable image styles, incorporating classes of object images in forms such as photographs, sketches, cartoons, paintings, product images, and etc. 
Correspondingly, current DG algorithms, which aim to learn domain invariant features out of the known domains, usually adapt domain shifts in between such arbitrarily decided image styles. 
We hereby present a newly designed DG dataset, SuperMarioDomains, containing four domains that are derived from four chronological titles in the Mario video game franchise on four generations of video game hardware. 
The discrepancy in between our domains is instead quantified in terms of progressively complex image representations that reflect the hardware evolution in image resolution, color palette, and presence of 3D rendering. 
We benchmark several state-of-the-art DG algorithms under both Multi-Source and Single-Source DG settings on SuperMarioDomains, and find our dataset possesses a decent challenge, much lower than other DG benchmarks.
We also propose a novel two-phase DG method MIRO2, showing that by incorporating our SuperMarioDomains dataset as part of tempering the pre-training process, we may receive state-of-the-art performances on existing Multi-Source DG benchmarks such as PACS and OfficeHome. 

==> draft/josh_idea.tex <==
Domain generalization is a fundamental challenge faced for the deployment of practical and safe machine learning algorithms. In classification specifically, learning discriminatory features requires significant consistency between examples of a given class. In real-world datasets, however, intra-class variation is high due to factors like lighting conditions, etc. This makes it difficult for models to differentiate between spurious and inherent features of classes, leading to inconsistent and potentially inflated performance.
\par
Simplified domains like those proposed in PACS [cite] (like sketch) offer a promising alternative for learning meaningful domain invariant features. By simplifying the domains to be represented, the models can better isolate shifts in the domain, improving their performance in generalization and robustness (cite: https://browse.arxiv.org/pdf/2201.00299.pdf). In PACS, however, classification is limited only to the salient objects of the image and representations of the same class in each domain are dramatically different both semantically (dog may refer to any breed of dog for instance) and stylistically (real word images are dramatically different from black and white sketches).
\par
Evolution in video game graphics, on the other hand, offer far more gradual shift. In each generation of Mario, designers have intended to draw similar scenes for their levels but were limited by hardware constraints. This setting provides a unique opportunity to observe how a human would stylistically compress a scene while preserving its inherent properties.
\par
Pre-training on our style shifted scenes improves performance when compared against real-world data pre-training datasets like ImageNet, despite the fact that the ImageNet images are far more similar to the test images than the Mario datset. This is highly significant and supports our claim that real-world domains are unsuitable for the initial construction of domain invariant features.

==> draft/new_abstract.tex <==
% In modern day computer vision applications, an ideally robust algorithm should be able to adapt to given environments, then perform good decision-making in unknown scenarios without additional supervision. Such domain generalization (DG) tasks require resources providing diverse simulated scenarios for which domain invariant features can be learned. Inspired by the evolving capability of video game graphics, we introduce SuperMarioDomains (SMD), a novel DG image classification dataset featuring images captured from multiple Mario games by Nintendo. Our dataset is split into four domains that are based on four generations of video game imagery with increasingly sophisticated graphics, ranging from heavily pixelated environments, to more vibrant scenarios in real-life-like colors and textures.Rather than focusing primarily on salient objects, our dataset challenges models to classify scenes corresponding to different Mario environments (i.e. Overworld, Underground, Aquatic, Castle). By benchmarking current State-of-the-Art image classification methods, we demonstrate that the task of DG on our dataset is significantly more challenging than existing DG benchmarks. Furthermore, we show that SuperMarioDomains is a superior pre-training data source for our proposed DG pre-training approach. Our proposed 2-phase domain generalization approach SMIRO may utilize the unique domain shift of holistic scenes found in SuperMarioDomains, and contributes to improvement performance on unseen target domains in several DG benchmarks. 

Domain generalization (DG) is a fundamental challenge for developing more robust machine learning algorithms. In image classification specifically, we require highly consistent examples of a given class in order to obtain domain-invariant features. However, current methods are often dependent on real-world image datasets with high intra-class variation e.g. ImageNet1K. Such dependency makes it difficult to extract inherent features of classes, potentially resulting in spurious correlation and inflated performance on DG benchmarks.
In this work, we introduce a new framework that focuses on more robust domain-invariant feature extraction. We curate SuperMarioDomains (SMD), a novel dataset consisting of simplified style-consistent domains and classes of synthetic scenes. We show that using SMD as precursor helps the state-of-the-art DG methods capture more holistic image features, and contributes to improved performance on unseen target domains in several DG benchmarks.  

==> figures/saliency_maps.tex <==

\begin{figure*}[h!]
\centering
\includegraphics[width=0.9\textwidth]{images/3-revised.png} 

\caption{Saliency maps produced by trained models from the baseline MIRO and the SMIRO$^{-}$ variants with alternative Oracle pre-training data, evaluated on the PACS benchmark. Red light regions are where each model focuses when predicting an unseen target domain image.}\label{figure1}
\label{saliency}
\end{figure*}


==> pages/11_smd_creation_details.tex <==

\begin{table}[t]
\centering
\small
\resizebox{\linewidth}{!}{
\begin{tabular}{@{}lrrrrrrr@{}}
\toprule
Console &Released in&Resolution &Color Palette&3D? \\\midrule
$\mathtt{NES}$ & 1985& 256×240 &50 colors&No\\
$\mathtt{SNES}$ &1990&512×478 &256 colors&No \\
$\mathtt{N64}$ &1996&704×480 &24-bit&Yes \\
$\mathtt{Wii}$ &2006&854×480 &32-bit&Yes \\
\bottomrule
\end{tabular}
}
\newline
\caption{Key graphical hardware specifications of the 4 Nintendo consoles, represented as the 4 domains in our SMD dataset. Images rendered on a newer-generation console generically reflect the console's strength to generate more complex shapes, more vibrant colors, and finer textures compared to its predecessor(s).}\label{tab: hardware}
\end{table}

% \begin{figure*}[ht!]
% \centering
% \includegraphics[width=\textwidth]{images/domain_comparison_2.png} 
% \caption{A close qualitative view of image domain discrepancy under a certain class in multiple DG datasets. Our domains are stratified by the evolving hardware capabilities of multiple game consoles referred in Table \ref{tab: hardware} over time. In PACS, the domains are differed by image styles: \textbf{P}hoto, \textbf{A}rt painting, \textbf{C}artoon, and \textbf{S}ketch. In VLCS, all images are real life photographs and the domains are simply the names of its 4 source collections: \textbf{V}OC2007 \cite{v}, \textbf{L}abelMe \cite{l}, \textbf{C}altech101 \cite{c}, and \textbf{S}UN09 \cite{s}. }
% \caption{A qualitative inspection over the designs of domains and classes in different DG datasets. \textbf{Left: }Domains in our dataset are based on diverse video game graphics rendered on different hardware. We classify the types of in-game holistic scenes for DG benchmarking. The scenes are labelled according to the environmental patterns and textures surrounding the player controlled Mario character at the center. \textbf{Right:} PACS' domains \cite{pacs} are distinct image styles - \textbf{P}hoto, \textbf{A}rt painting, \textbf{C}artoon, and \textbf{S}ketch. Its DG classification objective is to distinguish the one salient object often at the center of an image.}
% \todo[]{put color histogram here}
% \caption{An overview of RGB color distributions in DG benchmark datasets.}
% \label{overview}
% \end{figure*}



%you can remove this paragraph, seem redundant. 
%In this section, we describe how we design and construct our dataset. We then present our own Domain Generalization baselines using existing DG methods.

% \subsection{Design Choices}

\noindent\textbf{Design choices.} We design our \textbf{SuperMarioDomains (SMD)} dataset as a new MSDG benchmark. Unlike existing MSDG datasets such as PACS \cite{pacs} or OfficeHome \cite{officehome} whose main task is on classifying the primary salient object in an image of different image styles, we consider the whole scene in image as a classifiable entity and thus require methods to capture holistic domain-invariant visual features. Our dataset features synthesized video game scenes starting from pixelated mosaic 2D graphics in 50 colors, all the way to high polygon 3D graphics in 32-bit colors. Our domains of choice are sourced from video game footage captured on 4 chronological generations of video game consoles, all manufactured by Nintendo: The Nintendo Entertainment System ($\mathtt{NES} $) released in 1985, the Super Nintendo Entertainment System ($\mathtt{SNES} $) in 1990, the Nintendo 64 ($\mathtt{N64} $) in 1996, and the $\mathtt{Wii} $ in 2006. Correspondingly, we name our domains after these 4 game consoles. 

% \noindent\textbf{Domains represented by evolving hardware.} We name our image domains after the game consoles of our choice - $\mathtt{NES} $, $\mathtt{SNES} $, $\mathtt{N64} $, and $\mathtt{Wii} $. Table \ref{tab: hardware} lists down the hardware specifications of the chosen game consoles, spanning across 4 sequential generations. Scenes rendered on newer hardware represent stronger image processing capability - faster processing speed, dedicated GPUs, larger memory, higher output resolution, more vibrant colors, etc. In essence, newer games released on newer hardware over time enjoy stronger graphics hardware and less limited ability to more closely mimic sophisticated real-life scene. Previous datasets for image Domain Generalization do not put such transitioning of graphic quality into consideration - they either address solely the full-picture domain shift such as synthetic versus photorealistic \cite{syn2real}, or simply choose to incorporate apparently distinguishable image styles as domains such as photos versus oil paintings versus hand sketches, by sampling straight out of pre-existing vast image collections \cite{pacs, domainnet}. Our dataset employs a much more deliberately controlled visual domain discrepancy in design, pacing its domains in a more controlled distance from each other. With such design, we aim to challenge the robustness of current high performing DG approaches. 



\medskip\noindent\textbf{Contents of data.} For the actual scene contents, we choose gameplay footages entirely from the Mario franchise, one title per our featured game consoles. The reason we decide to use the Mario games is that the Mario franchise has a consistent level and scenery design shared across generations, and hence we may be able to apply consistent scene labels regardless the evolution of visual quality. Respectively, our dataset incorporates gameplay footage from \textit{Super Mario Bros} on $\mathtt{NES} $, \textit{Super Mario World} on $\mathtt{SNES} $, \textit{Mario 64} on $\mathtt{N64} $, and \textit{Super Mario Galaxy} on $\mathtt{Wii} $ - the former two games rendered in 2D graphics while the latter two in 3D. 

\medskip\noindent\textbf{Defining scene classes.} For the scene labels for image classification, we land on 4 classes of distinct in-game scenes that consistently appear in all Mario games of our choice. Each scene class has its own unique traits defined by the combination of terrains, objects, and colors. We use the following rules as our manual annotation guidelines: 
\begin{itemize}[noitemsep, nosep]
    \item \textbf{Overworld} scenes cover a wide range of outdoors levels with an open background and natural green vegetation, such as grassland or forest. 
    \item \textbf{Underground} scenes feature closed-off dark interior background with sporadic weak lighting and mountain cave, ice cave, or sewage textures.
    \item \textbf{Aquatic} scenes appear with watery textures surrounded by aquatic creatures such as fish or squid, and oftentimes with swimming movements by the player controlled character. 
    \item \textbf{Castle} 
    %or `Boss Fight' %
    scenes 
    %are stages within 
    have dungeon-like environments, normally indoors and/or with an architectural texture and rampant gimmicky obstacles such as traps and spikes.
\end{itemize}


\medskip\noindent\textbf{Dataset construction.} We sample our images from public game play videos uploaded to YouTube and Twitch.tv. We use video recordings in the highest quality (1080p HD, 60 frames per second) that cover all the levels in games from start to end as to include as many diverse scenes as possible. We employ a group of three persons who are all familiar with the featured games for data annotation. 
We label the in-game scenes by segmenting the video footage, so that all consistent frames within one scene segment share the same scene label. 
%We skip the segments that do not depict any level designs, such as those when narrative stories are played, the scoreboard is displayed, or the whole screen is blackened out for level transition. 
We then down-sample every labeled video segment. We sample evenly-spaced frames from $\mathtt{NES} $ and $\mathtt{SNES} $ video segments at a higher 10 fps, while we sample at a lower 3 fps from $\mathtt{N64} $ and $\mathtt{Wii} $ segments.  We also crop out the on-screen texts, the user interface, and the level floor regions from each individual image frame, so that we include less heuristic bias from scene-specific artifacts. Eventually, we yield 7K samples for $\mathtt{NES}$, 20K for $\mathtt{SNES}$, 25K for $\mathtt{N64}$, and 30K for $\mathtt{Wii}$ for the SMD dataset, and each scene class has the same number of images per domain.

\input{pages/11a_datasetstats}

% After manual inspection by removing any mislabeled, duplicate, or pure-color images, we conduct integrity check of our dataset by verifying our 4 scene classes are all separable within the scope of each domain. With a training-test split ratio of 8 to 2 for each domain, the in-domain test accuracies reach above 96\% with regard to all domains \hl{by training a simple image classifier of a ResNet18 backbone followed by a linear classifier from scratch}. We eventually yield 7K samples for $\mathtt{NES}$, 20K for $\mathtt{SNES}$, 25K for $\mathtt{N64}$, and 30K for $\mathtt{Wii}$. Within each individual domain, each scene class has the same number of samples. Examples from our dataset are shown in Figure \ref{overview} on the Left. 

% \begin{wraptable}{r}{0.5\textwidth} 
% \centering
% \vspace{-22pt}
% \caption{The in-domain test accuracy using basic classification models from scratch. \\ }\label{tab: in-domain}
% \small
% \begin{tabular}{lrrrrr}\toprule
% Model &NES &SNES &N64 &Wii \\\midrule
% Resnet18 &99.1 &96.3 &97.9 &98.9 \\
% Resnet50 &99.0 &96.2 &98.3 &98.6 \\
% \bottomrule
% \end{tabular}
% \end{wraptable}

% Eventually, our dataset consists of debiased gameplay video frames of 4 domains and 4 scene classes. 

% The source video length for each domain increases by generation: the most aged NES domain has the fewest possible unique frames from less than 1 hour of gameplay, while the latest Wii domain are down-sampled from 10 hours of recordings. 




==> pages/11a_datasetstats.tex <==
\begin{table}[t]
\centering
\small
% \begin{tabular}{lrrrr}\toprule
% Domain &Overworld &Underground &Aquatic &Castle \\\midrule
% NES &10K &3.4K &5K &3.6K  \\
% SNES &17K &8K &4K &6K  \\
% N64 &30K &7K &6K &7K  \\
% Wii &61K &19K &23K &18K \\
% \bottomrule
% \end{tabular}
% \newline
% \caption{The numbers of raw scene samples. The 4 classes of labeled scenes back in the original gameplay videos are distributed disproportionately. So we further down-sample them evenly and make sure each domain shares the same number of the samples per label.\\}\label{tab: stats}

\begin{tabular}{lllr}\toprule
Benchmark & Domains & Classes &  Size  \\\midrule
PACS \cite{pacs}& 4 image styles & 7 objects &10K   \\
VLCS \cite{vlcs}& 4 photo sources & 5 objects &10K    \\
TerraIncognita \cite{terraincongnita} & 4 locations & 10 animals & 25K \\
OfficeHome \cite{officehome}&4 image styles &65 objects &16K   \\
Syn2real-C \cite{syn2real}&real \& rendered &12 objects &280K   \\
DomainNet \cite{domainnet}&6 image styles &345 objects &587K  \\
\midrule
SMD (ours)& 4 game graphics & 4 scenes& 82K \\
\bottomrule
\end{tabular}
\newline
\caption{Statistics of popular image classification datasets for MSDG. While ours does not stand out in scale, we introduce the challenge of classifying holistic scenes instead of salient objects, across domains of distinct video game graphics. }\label{tab: stats_dataset}
\end{table}

==> pages/12_mariodgbaseline.tex <==
\subsection{MSDG Baselines of SuperMarioDomains} 
\label{chap: mario-baselines}

\input{pages/06__1_smd_benchmark_results}

% \textbf{Experiment setups.} We deploy ResNet50 \cite{resnet} as the default backbone, optionally with the pre-trained weights from ImageNet1K \cite{imagenet}. We also experiment with a larger-scale backbone, RegNetY-16GF \cite{regnet}, with possible pre-trained weights by the weakly supervised SWAG \cite{swag} over 3.6B noisy Instagram images.  

% \noindent\textbf{SMD baselines.} 

Table \ref{tab: mario-baselines} demonstrates the performances from the current top performing non-ensemble DG methods on our dataset. We observe the MSDG task becomes increasingly harder as the unseen target domain features more complex scene graphics from 2D to 3D. Targeting the least complex $\mathtt{NES}$ domain can be as high as $+40.4\%$ above random by CDANN, while targeting the most complex $\mathtt{Wii}$ domain is $+8.5\%$ above random at best by DANN. Similarly, generalization targeting the combined two $\mathtt{2D}$ domains as a whole is easier than that targeting two $\mathtt{2D}$ domains; the former can be as high as $+28.0\%$ above random by CDANN, while the latter is $+7.0\%$ at best by MTL. In general, SMD shows its unique difficulty from a universal trend by all observed DG methods: the MSDG performance deteriorates as the unseen target domain becomes more graphically evolved.

% In the latter part of Table \ref{tab: mario-baselines} featuring the RegNetY-16GF backbone, we witness more irregularities even with roughly 40 times more trainable parameters. ERM and SagNet display similar performance with those of the ResNet50 backbone, as well as the similar outcomes that the scratch backbone over-performs the pre-trained backbone. RandConv displays alternating outcomes with and without SWAG pre-training. MIRO, now equipped with the large backbone, enjoys the overall best DG result on Mario of 48.3\% but \textit{with} pre-training, beating its scratch backbone counterpart by +5.3\% (43.0\% $\rightarrow$ 48.3\%) and surpassing the ResNet50 baseline by a small margin of +2.6\% (45.7\% $\rightarrow$ 48.3\%). Still, when compared to performances on other DG benchmarks by MIRO, the current top baselines of our SMD dataset are still relatively low with both ResNet50 and RegNetY-16GF backbones.  





% \yiranresponse{TODO }

==> pages/13_smd_benchmark_results.tex <==
\begin{table}[!t]\centering

\small
\resizebox{\linewidth}{!}{
\begin{tabular}{l|rrrr|rr}\toprule
\multirow{2}{*}{\textbf{Method}}& \multicolumn{6}{c}{SMD Target Domain(s)}  \\
&$\mathtt{NES}$&$\mathtt{SNES}$& $\mathtt{N64}$& $\mathtt{Wii}$ &$\mathtt{2D}$&$\mathtt{3D}$ \\ \midrule
Random &25.0 &25.0 &25.0 &25.0 &25.0 &25.0\\
\midrule
% RandConv \cite{randconv}        &40.5 &34.0 &22.2 &25.0 &30.4 \\
ERM \cite{gulrajani2021in}      &46.7 &36.4 &23.5 &26.0     &39.8 & 30.6\\
SagNet \cite{sagnet}            &43.7 &38.4 &26.1 &28.5     &37.8 &29.3\\
Mixstyle \cite{mixstyle2021}    &47.3 &36.2 &\textbf{33.0}  &27.7   &49.8 &27.5\\
GroupDRO \cite{groupdro2020}    &50.6 &38.4 &25.7 &30.0     &37.4 & 29.7\\
MLDG  \cite{mldg}               &52.0 &41.0 &24.5 &28.7     &35.5 & 31.1\\
MIRO  \cite{miro}               &50.9 &42.6 &24.7 &28.9     &42.1 & 30.8\\
MTL   \cite{mtl}                &51.0 &36.1 &30.5 &30.2     &40.5 & \textbf{32.0}\\
IRM \cite{irm2022}             &45.5 &44.9 &27.1 &32.7      &41.0 & 27.8\\
VREx \cite{VREx}                &55.6 &39.0 &26.0 &30.8     &35.2 &30.1 \\
CORAL \cite{coral2016}          &59.4 &43.0 &30.0 &31.3     &38.1 & 30.7\\
Mixup \cite{mixup}              &62.8 &43.7 &28.0 &29.7     &40.8 & 30.6\\
ARM \cite{arm2021}              &61.7 &47.6 &26.9 &30.4     &44.6 & 29.7\\
RSC \cite{rsc}                  &64.6 &44.5 &29.1 &28.5     &44.5 & 28.5\\
DANN \cite{dann}                &57.7 &58.7 &29.1 &\textbf{34.5}            &52.9 &31.3\\
CDANN \cite{cdann}              &\textbf{65.4} &\textbf{67.8} &28.3 &28.4   &\textbf{53.0} &31.3\\
% & & & & & \\
% In-domain &99.0 &97.0 &98.0 &97.0 &97.8 \\
\bottomrule
\end{tabular}
}
\caption{MSDG cross-validation baselines of SMD by methods that use ResNet50 as the only feature extracting backbone. One single target domain, e.g. $\mathtt{NES}$, indicates the source domains are the remaining $\mathtt{SNES}$, $\mathtt{N64}$ and $\mathtt{Wii}$ combined. Target domain $\mathtt{2D}$ stands for $\mathtt{NES}+\mathtt{SNES}$, and $\mathtt{3D}$ stands for $\mathtt{N64}+\mathtt{Wii}$. The \textbf{best results} by each target domain category are highlighted in bold. All results are averaged over 3 trials within an error range of $\pm 0.5$.}
 \vspace*{-0.7\baselineskip}
\label{tab: mario-baselines}
\end{table}

% \begin{table*}[!h]\centering

% \footnotesize
% \begin{tabular}{l|r|rrrr|rr}\toprule
% \multirow{2}{*}{\textbf{Algorithm}}& \multirowcell{2}{Pre-trained \\ backbone}& \multicolumn{4}{c|}{SMD Test Set Domain} & \\
% &&NES &SNES &N64 &Wii &Avg.& $\Delta$ \\ \midrule
% Random &- &25.0\err{0.0} &25.0\err{0.0} &25.0\err{0.0} &25.0\err{0.0} &25.0\err{0.0} &0.0\\
% \midrule
% \multicolumn{7}{l}{\textit{Using ResNet50 backbone with possible ImageNet1K pre-training, 47M parameters.}}\\
% \midrule

% ERM&\multicolumn{1}{l|}{\cmark} &46.7\err{1.2} &36.4\err{1.8} &23.5\err{1.3} &26.0\err{1.6} &33.2\err{1.1}&+8.2 \\
% &\xmark &50.6\err{1.0} &54.9\err{1.6} &32.2\err{1.1} &28.7\err{0.8} &41.6\err{0.7}& +16.6\\
% SagNet &\multicolumn{1}{l|}{\cmark}  &43.7\err{1.3} &38.4\err{1.4} &26.1\err{1.2} &28.5\err{1.3} &34.2\err{0.9}& +9.2\\
% &\xmark &55.1\err{1.0} &53.2\err{0.9} &32.1\err{0.7} &28.7\err{0.4} &42.3\err{0.8}& +19.3\\
% RandConv&\multicolumn{1}{l|}{\cmark}  &40.5\err{1.2} &34.0\err{1.4} &22.2\err{2.2} &25.0\err{1.1} &30.4\err{1.5}&+5.4 \\
% &\xmark &51.6\err{0.8} &50.8\err{1.5} &30.9\err{1.0} &26.7\err{1.2} &40.0\err{1.1}&+15.0 \\
% MIRO&\multicolumn{1}{l|}{\cmark}  &50.9\err{0.6} &42.6\err{0.9} &24.7\err{0.9} &28.9\err{0.5} &36.8\err{0.8}& +11.8\\
% &\xmark &\textbf{64.3}\err{0.6} &\textbf{56.2}\err{0.7} &\textbf{33.4}\err{1.0} &\textbf{29.2}\err{0.6} &\textbf{45.7}\err{0.9}& \textbf{+20.7}\\
% \midrule
% \multicolumn{7}{l}{\textit{Using RegNetY-16GF backbone with possible SWAG pre-training, 1.6B parameters.}}\\
% \midrule
% ERM &\multicolumn{1}{l|}{\cmark}  &46.5\err{0.5} &37.6\err{0.0} &21.6\err{0.3} &28.4\err{0.4} &33.5\err{0.2} &+8.5\\
% &\xmark &54.0\err{1.1} &51.3\err{1.9} &29.4\err{0.7}&29.1\err{0.1}&41.0\err{0.6}&+16.0\\
% SagNet &\multicolumn{1}{l|}{\cmark}  &44.0\err{0.3} & 36.5\err{1.2} &21.0\err{0.2} & 26.1\err{0.8} & 31.9\err{0.9} &+6.9\\
% &\xmark &49.1\err{1.8} &51.7\err{1.1} &33.7\err{0.3} &29.1\err{1.3} &40.9\err{1.0} &+15.9\\
% RandConv &\multicolumn{1}{l|}{\cmark}  &47.5\err{0.7} &56.3\err{0.1} &\textbf{43.7}\err{0.2} &25.5\err{0.3} &43.3\err{0.4} &+18.3\\ 
% &\xmark &43.1\err{0.7} &57.1\err{0.5} &32.0\err{1.0} &28.0\err{1.1} &40.1\err{0.8}&+15.1 \\
% MIRO &\multicolumn{1}{l|}{\cmark}  &\textbf{63.5}\err{0.1} &\textbf{65.0}\err{0.5} &32.3\err{0.7} &\textbf{32.4}\err{0.7} &\textbf{48.3}\err{0.7}&\textbf{+23.3}\\
% &\xmark & 52.8\err{1.4}&54.4\err{1.2} &37.0\err{0.5} &28.4\err{1.0} &43.2\err{1.2}&+18.2 \\
% \bottomrule
% \end{tabular}
% \caption{The indigenous baselines of Multi-Source Domain Generalization on the SMD dataset with existing top-performing DG algorithms. The \textbf{best results} are highlighted in bold per backbone. $\Delta$ indicates the best average improvement over the random baseline. All average accuracies and errors are reported from three trials. 
% }
% % \todo{why is SMIRO, SMIRO+KL (Ours) missing here? }
% % \yiranresponse{L: The baselines are from existing DG methods. Also, SMIRO would use Mario itself to train the oracle, then perform DG on Mario for testing. This is like running Mario benchmarks on a Mario-pretrained model.}
% % \todo{why are Sagnet and RandConv not implemented with RegNetY-16GF backbone. }
% % \yiranresponse{L: The sota framework only reported ERM and MIRO for Regnet backbone. But I actually have those results as well. Will be attached.}
% \label{tab: mario-baselines}
% \end{table*}
\input{pages/06__2_oracle_pretrain_results_table}
